Field- and damping-like spin-transfer torque in magnetic multilayers

We investigate the spin-transfer torque in a magnetic multilayer structure by means of a spin-diffusion model. The torque in the considered system, consisting of two magnetic layers separated by a conducting layer, is caused by a perpendicular-to-plane current. We compute the strength of the field-like and the damping-like torque for different material parameters and geometries. Our studies suggest that the field-like torque highly depends on the exchange coupling strength of the itinerant electrons with the magnetization both in the pinned and the free layer. While a low coupling leads to very high field-like torques, a high coupling leads to low or even negative field-like torques. The dependence of the different torque terms on system parameters is considered very important for the development of applications such as STT MRAM and spin-torque oscillators.

==> translator-language-mappings.tex <==
% Copyright 2007 by Till Tantau
% Copyright 2010 by Vedran Mileti\'c
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the documentation file for more details.

\def\trans@use@and@alias#1#2{%
  \uselanguage{#2}%
  \languagealias{#1}{#2}%
}

\DeclareOption{acadian}        {\trans@use@and@alias{french}    {Acadian,French}}
\DeclareOption{afrikaans}      {\trans@use@and@alias{afrikaans} {Afrikaans,Dutch}}
\DeclareOption{american}       {\trans@use@and@alias{american}  {AmericanEnglish,English}}
\DeclareOption{austrian}       {\trans@use@and@alias{austrian}  {Austrian1997,Austrian,German1997,German}}
\DeclareOption{bahasa}         {\trans@use@and@alias{bahasa}    {Bahasa}}
\DeclareOption{basque}         {\trans@use@and@alias{basque}    {Basque}}
\DeclareOption{brazil}         {\trans@use@and@alias{brazil}    {Brazilian,Portuguese}}
\DeclareOption{brazilian}      {\trans@use@and@alias{brazilian} {Brazilian,Portuguese}}
\DeclareOption{breton}         {\trans@use@and@alias{breton}    {Breton}}
\DeclareOption{british}        {\trans@use@and@alias{british}   {BritishEnglish,English}}
\DeclareOption{bulgarian}      {\trans@use@and@alias{bulgarian} {Bulgarian}}
\DeclareOption{canadian}       {\trans@use@and@alias{canadian}  {Canadian,English}}
\DeclareOption{canadien}       {\trans@use@and@alias{canadien}  {Canadien,French}}
\DeclareOption{catalan}        {\trans@use@and@alias{catalan}   {Catalan}}
\DeclareOption{croatian}       {\trans@use@and@alias{croatian}  {Croatian}}
\DeclareOption{czech}          {\trans@use@and@alias{czech}     {Czech}}
\DeclareOption{danish}         {\trans@use@and@alias{danish}    {Danish}}
\DeclareOption{dutch}          {\trans@use@and@alias{dutch}     {Dutch}}
\DeclareOption{english}        {\trans@use@and@alias{english}   {English}}
\DeclareOption{esperanto}      {\trans@use@and@alias{esperaton} {Esperanto}}
\DeclareOption{estonian}       {\trans@use@and@alias{estonian}  {Estonian}}
\DeclareOption{finnish}        {\trans@use@and@alias{finnish}   {Finnish}}
\DeclareOption{francais}       {\trans@use@and@alias{french}    {French}}
\DeclareOption{frenchb}        {\trans@use@and@alias{french}    {French}}
\DeclareOption{french}         {\trans@use@and@alias{french}    {French}}
\DeclareOption{galician}       {\trans@use@and@alias{galician}  {Galician}}
\DeclareOption{german}         {\trans@use@and@alias{german}    {German1997,German}}
\DeclareOption{germanb}        {\trans@use@and@alias{german}    {German1997,German}}
\DeclareOption{greek}          {\trans@use@and@alias{greek}     {Greek}}
\DeclareOption{polutonikogreek}{\trans@use@and@alias{greek}     {Polutoniko,Greek}}
\DeclareOption{hebrew}         {\trans@use@and@alias{hebrew}    {Hebrew}}
\DeclareOption{hungarian}      {\trans@use@and@alias{hungarian} {Hungarian}}
\DeclareOption{icelandic}      {\trans@use@and@alias{icelandic} {Icelandic}}
\DeclareOption{irish}          {\trans@use@and@alias{irish}     {Irish}}
\DeclareOption{italian}        {\trans@use@and@alias{italian}   {Italian}}
\DeclareOption{latin}          {\trans@use@and@alias{latin}     {Latin}}
\DeclareOption{lowersorbian}   {\trans@use@and@alias{lsorbian}  {LowerSorbian,Sorbian}}
\DeclareOption{magyar}         {\trans@use@and@alias{magyar}    {Magyar}}
\DeclareOption{naustrian}      {\trans@use@and@alias{naustrian} {Austrian,German}}
\DeclareOption{ngerman}        {\trans@use@and@alias{ngerman}   {German}}
\DeclareOption{norsk}          {\trans@use@and@alias{norsk}     {Norsk}}
\DeclareOption{samin}          {\trans@use@and@alias{samin}     {Samin}}
\DeclareOption{nynorsk}        {\trans@use@and@alias{nynorsk}   {Nynorsk,Norsk}}
\DeclareOption{polish}         {\trans@use@and@alias{polish}    {Polish}}
\DeclareOption{portuges}       {\trans@use@and@alias{portuges}  {Portuguese}}
\DeclareOption{portuguese}     {\trans@use@and@alias{portuguese}{portuguese}}
\DeclareOption{romanian}       {\trans@use@and@alias{romanian}  {Romanian}}
\DeclareOption{russian}        {\trans@use@and@alias{russian}   {Russian}}
\DeclareOption{scottish}       {\trans@use@and@alias{scottish}  {Scottish}}
\DeclareOption{serbian}        {\trans@use@and@alias{serbian}   {Serbian}}
\DeclareOption{slovak}         {\trans@use@and@alias{slovak}    {Slovak}}
\DeclareOption{slovene}        {\trans@use@and@alias{slovene}   {Slovene}}
\DeclareOption{spanish}        {\trans@use@and@alias{spanish}   {Spanish}}
\DeclareOption{swedish}        {\trans@use@and@alias{swedish}   {Swedish}}
\DeclareOption{turkish}        {\trans@use@and@alias{turkish}   {Turkish}}
\DeclareOption{ukrainian}      {\trans@use@and@alias{ukrainian} {Ukrainian}}
\DeclareOption{uppersorbian}   {\trans@use@and@alias{usorbian}  {UpperSorbian,Sorbian}}
\DeclareOption{welsh}          {\trans@use@and@alias{welsh}     {Welsh}}
\DeclareOption{UKenglish}      {\trans@use@and@alias{UKenglish} {BritishEnglish,English}}
\DeclareOption{USenglish}      {\trans@use@and@alias{USenglish} {AmericanEnglish,English}}
\ProcessOptions*

